Missing Data Imputation and Acquisition with Deep Hierarchical Models and Hamiltonian Monte Carlo

Variational Autoencoders (VAEs) have recently been highly successful at imputing and acquiring heterogeneous missing data. However, within this specific application domain, existing VAE methods are restricted by using only one layer of latent variables and strictly Gaussian posterior approximations. To address these limitations, we present HH-VAEM, a Hierarchical VAE model for mixed-type incomplete data that uses Hamiltonian Monte Carlo with automatic hyper-parameter tuning for improved approximate inference. Our experiments show that HH-VAEM outperforms existing baselines in the tasks of missing data imputation and supervised learning with missing features. Finally, we also present a sampling-based approach for efficiently computing the information gain when missing features are to be acquired with HH-VAEM. Our experiments show that this sampling-based approach is superior to alternatives based on Gaussian approximations.

==> old_introduction.tex <==

\section{Introduction}
\label{sec:intro}

Variational Autoencoders \citep{kingma2013auto, rezende2014stochastic, kingma2019introduction} stand out in the recent literature as robust generative models that efficiently handle high-dimensional data. In their naive configuration, every data dimension is assumed to have similar statistical properties (i.e., homogeneity), and all dimensions are considered to be completely observed. Both assumptions are far from  reality in many real-world applications where different data types (real, positive-valued, continuous, or discrete) coexist within the same dataset and the collected data might be partially observed. Recent works have successfully adapted VAEs to handle incomplete \citep{collier2020vaes, ma2018eddi, garnelo2018conditional, mattei2019miwae} and mixed-type data \citep{nazabal2020handling, ma2020vaem, gong2021variational}. Based on these models, efficient algorithms have been derived for downstream tasks, including: 1) missing data imputation; 2) supervised learning with missing data; 3) sequential active information acquisition.
%, which is important in cost-sensitive applications.
%3), outlier identification, typically handled by evaluating the likelihood \citep{eduardo2020robust, klambauer2017self}. 
Despite these advances, existing approaches are restricted by using only one layer of latent variables, which reduces flexibility; 
and Gaussian posterior approximations, which introduce inference bias. These design choices limit performance in real-world settings with complex mixed-type incomplete data.

Bias can be reduced by using Monte Carlo sampling instead of  Gaussian-based approximations \citep{salimans2015markov, thin2021monte}. In \citep{hoffman2017learning}, the authors propose to initialize a Markov Chain Monte Carlo (MCMC) method %\citep{neal1993probabilistic} 
with proposals given by the variational approximation provided by the Gaussian encoder, achieving higher likelihoods and producing samples with better quality. 
%More specifically, 
Hamiltonian Monte Carlo (HMC) \citep{duane1987hybrid, betancourt2015hamiltonian} stands out among MCMC methods in machine learning
due to its superior efficiency for exploring regions of interest in the target density. In \citep{caterini2018hamiltonian}, HMC is combined with stochastic variational inference for improving the training of VAEs. Motivated by the strong influence that hyperparameters have in the performance of HMC, \citep{campbell2021gradient} describes an  automatic framework for tuning the HMC hyper-parameters in VAEs by optimizing a tractable objective with SGD. %However, 

All the previous works consider only VAEs with only one layer of latent variables and 
homogeneous data. %None of them has been adapted to either hierarchical VAEs or the presence of mixed-type data.
Modeling flexibility can be increased by considering hierarchical VAEs with
multiple layers of hidden variables \citep{sonderby2016ladder, maaloe2019biva, vahdat2020nvae, child2020very}. These models have become highly influential recently  because of the high quality of their samples.
%ir success in incorporating effective inductive biases and enriching the resulting prior over latent variables. 
By using a hierarchical structure in the latent space, they enforce the information to flow from high-level representations to more specific observable factors, imitating the way information is often organized in the real world. However, the hierarchical organization of the latent variables creates complicated posterior dependencies that are not straightforward to deal with and require special consideration. To improve Gaussian approximate inference, most  works opt by defining shared paths between the recognition and generative networks.
While this makes hierarchical VAEs practical, the bias introduced by the Gaussian approximations is still present.
%Furthermore, the curse of dimensionality increases the looseness of the variational bound caused by the Gaussian approximation. Adding autoregressive latent variables implies an expansion of the latent space, which has a similar effect to increasing the latent dimensionality. 
%In this work, we incorporate and tune HMC to a hierarchical generative model to address the looseness of the Gaussian approximation bound and enhance the optimization of the generative networks. 
To the best of our knowledge, none of the aforementioned hierarchical VAEs has been previously combined with Monte Carlo algorithms for improving over standard Gaussian approximate inference.

To overcome such limitations, we focus on training new hierarchical VAE models 
for heterogeneous mixed-type data with
HMC. Our models can be used for missing data imputation and for supervised learning with missing data.
%and outlier identification. 
We also present a sampling-based  framework that allows our models to perform accurate sequential active information acquisition.

Our main contributions are as follows:
\begin{itemize}
    \item We present HH-VAEM, a deep hierarchical model for handling mixed-type incomplete data that uses HMC with automatic hyper-parameter tuning for outperforming amortized variational inference by generating low bias samples from the true posterior. %To our knowledge, our work is the first that incorporates unbiased inference in hierarchical VAEs and, further, generalises to the mixed-type incomplete data condition.
    \item We propose a sampling-based strategy for missing feature acquisition that benefits from the improved inference of HH-VAEM. %We demonstrate its superiority with respect to the Gaussian-based approaches in the task of sequentially collecting variables.
    By using histograms to estimate the mutual information, this strategy achieves lower bias than other Gaussian-based alternatives.
    \item We exhaustively evaluate HH-VAEM in the tasks of 1) missing data imputation, 2) supervised learning with missing data and 3)
    information acquisition
    with our sampling-based strategy. In all cases we report significant gains with respect to baselines.
\end{itemize}

